Follow-on Question Suggestion via Voice Hints for Voice Assistants

The adoption of voice assistants like Alexa or Siri has grown rapidly, allowing users to instantly access information via voice search. Query suggestion is a standard feature of screen-based search experiences, allowing users to explore additional topics. However, this is not trivial to implement in voice-based settings. To enable this, we tackle the novel task of suggesting questions with compact and natural voice hints to allow users to ask follow-up questions. We define the task, ground it in syntactic theory and outline linguistic desiderata for spoken hints. We propose baselines and an approach using sequence-to-sequence Transformers to generate spoken hints from a list of questions. Using a new dataset of 6681 input questions and human written hints, we evaluated the models with automatic metrics and human evaluation. Results show that a naive approach of concatenating suggested questions creates poor voice hints. Our approach, which applies a linguistically-motivated pretraining task was strongly preferred by humans for producing the most natural hints.

==> limitations.tex <==
\section{Limitations and Future Work}\label{sec:limitations}

\noindent\change{\textbf{Languages.} In this paper, we limited our work only the English language for obtaining training and testing data for generating voice-friendly hints. As a next step, we foresee adding other languages, such as German, Korean, and Chinese, and understanding the implications in terms of the required syntactic and semantic operations to generate hints that are voice-friendly.}

\noindent\change{\textbf{Scenarios:} Our work focused only on a single turn conversations, where after a user asks a question to a voice assistant, a hint suggesting questions about related topics to the user's initial question are uttered back to the user. Future steps include multi-turn conversations, where user interests and actions after each hint will impact the generated hints for follow-up turns. There are several strategies that can be considered, and we aim at investigating the following: dive deeper in a topic of user's interest (suggest more targeted questions on a specific topic about the entity of interest), or broaden user's knowledge on a given topic (i.e., suggest questions about \emph{related entities}).}

\noindent\textbf{Training and Evaluation:} As future work we foresee integrating more targeted training and modelling strategies that aim at better integrating complex and erroneous questions into the hint. Additionally, we aim at designing more human evaluation studies, where we assess how correlated are follow-up questions  with the suggested questions in a hint.

